DynamiQ: Planning for Dynamics in Network Streaming Analytics Systems

The emergence of programmable data-plane targets has motivated a new hybrid design for network streaming analytics systems that combine these targets' fast packet processing speeds with the rich compute resources available at modern stream processors. However, these systems require careful query planning; that is, specifying the minute details of executing a given set of queries in a way that makes the best use of the limited resources and programmability offered by data-plane targets. We use such an existing system, Sonata, and real-world packet traces to understand how executing a fixed query workload is affected by the unknown dynamics of the traffic that defines the target's input workload. We observe that static query planning, as employed by Sonata, cannot handle even small changes in the input workload, wasting data-plane resources to the point where query execution is confined mainly to userspace. This paper presents the design and implementation of DynamiQ, a new network streaming analytics platform that employs dynamic query planning to deal with the dynamics of real-world input workloads. Specifically, we develop a suite of practical algorithms for (i) computing effective initial query plans (to start query execution) and (ii) enabling efficient updating of portions of such an initial query plan at runtime (to adapt to changes in the input workload). Using real-world packet traces as input workload, we show that compared to Sonata, DynamiQ reduces the stream processor's workload by two orders of magnitude.

==> background.tex <==
\section{Background and Motivaton}
\label{sec:background}
Sonata~\cite{sonata} lets network operators express network monitoring tasks as dataflow queries over packet fields, without worrying about where and how these queries get executed. In this section, we first present how Sonata uses raw packet traces from the network to compute query plans, and then describe why it fails to handle traffic dynamics. 


\begin{figure*}[t] 
\centering
\resizebox{.4\linewidth}{!}{
\includegraphics[trim=125 450 550 0]{drawings/dynaso_background.pdf}}
\caption{Relationship between workload at the switch and the load at the stream processor for Sonata. 
\label{fig:sonata-arch}} 
\ifx \compress \undefined
\else
\vspace*{-1\baselineskip}
\fi
\end{figure*}


\subsection{Sonata's Query Planning}

 
% \begin{figure}[t!]
% \begin{lstlisting}[language=query2,basicstyle=\footnotesize, 
% basicstyle=\footnotesize, numbers=left,xleftmargin=2em,frame=single,
% framexleftmargin=2.0em, captionpos=b, label=tcp-conn, 
% caption=Detect Newly Opened TCP Connections~\cite{sonata-github}.]
% packetStream(W)
% .filter(p => p.tcp.flags == 2)
% .map(p => (p.dIP, 1))
% .reduce(keys=(dIP,), f=sum)
% .filter((dIP, count) => count > Th)
% \end{lstlisting}
% \ifx \compress \undefined
% \else
% \vspace*{-1\baselineskip}
% \fi
% \end{figure}
 
% \paragraph{Key ideas}


%\paragraph{Goal.}


\paragraph{Packet traces to cost matrices.}
To compute the query plan, Sonata's query planner divides the input packet traces into multiple (three second) windows. For each window, it generates a cost matrix. Each element in this cost matrix is a tuple ($B_{q,i,j,k},  N_{q,i,j,k}$), where $B$ is the amount of stateful memory required, and $N$ is the number of output packets (tuples) for the $k^{th}$ operator of query $q$ at refinement level $j$ after executing at level $i$. To compute the value of this tuple for a window, Sonata's query planner synthesizes a version of the input query such that it executes the query $q$ till the $k^{th}$ operator at refinement level $j$ after executing the query at at level $i$ and runs it over the raw packet traces collected for that window. Clearly, as generating cost matrices requires executing input queries for all possible combinations of refinement and partitioning plans, it is computationally intense. More cocnretely, if, $Q$, $R$ and $P$ represent the set of queries, refinement levels and stateful operators, respectively, then the total number of queries it needs to run to generate the cost matrix are $\frac{|Q||R||R-1||P|}{2}$. Even with the state-of-the-art data analytics system, BigQuery~\cite{bigquery}, computing cost matrix for a single window takes XX hours. 

% \ag{TODO: make it clear that given the overhead of computing cost matrices, we should only expect their limited availability.}

\paragraph{Cost matrices to query plans.}
Sonata relies on two key ideas to scale flexible streaming queries. First, it partitions the query between the data-plane (switch) and a user-space (stream processor) targets. Second, it dynamically refines the input queries to zoom-in on traffic of interest over time. Each Sonata query is an ordered set of dataflow operators such as a {\tt map}, {\tt reduce}, {\tt filter}, etc. Sonata makes the decision to partition these ordered sets of operators into two disjoint sets: one set that it executes in the data plane and the other that it executes in the user space (using a stream processor). Similarly, for the hierarchical keys (such as DNS names, ipv4 addresses), etc., it decides a sequence of refinement levels, i.e., the refinement plan. 

After computing the cost matrices for multiple windows, Sonata's query planner then feeds the median value of the cost matrices as input to an integer linear program (ILP), which takes various data-plane and ordering constraints into consideration to compute the query plan that minimizes the number of packets sent to the stream processor. More concretely, it takes the following four switch constraints into consideration for query planning: M--the amount of metadata stored in the switch, A--the number of stateful actions per stage, B--register memory in bits per stage, S--the number of stages in match action pipeline. 

\ag{Note: I have merged partitioning and mapping decisions together, which makes more sense to me. Operators that do not find a match in the data plane are implicitly mapped to the stream processor.}

We can divide Sonata's query-planning decisions into three categories: (1)~{\em refinement plan}, i.e., a sequence of refinement levels for stateful operators with hierarchical keys (such as DNS names, ipv4 addresses), etc.; (2)~{\em hash-table sizing}, i.e., deciding how much memory to allocate to each hash table for stateful operations in the data plane; and (3)~{\em operator mapping}, i.e., which decides whether to execute a stateful operator in the data plane or stream processor. For all the operators it decides to execute in the data plane, it needs to determine mapping of these operators to has tables in the data plane.  




\subsection{Handling Workload Dynamics}
\label{ssec:query-planning-challenges}

\paragraph{Sonata's query planner's assumptions.}
As we discussed earlier, Sonata uses historical packet traces to determine the query plan. Sonata assumed that given that the workload at the switch, i.e., the total number of incoming packets at the switch, as well as the corresponding workload for the query plan, i.e., cost matrices do not change much over time. As a result, the query plan it trained using the historical data should work well in the future as well. Our results show that this assumption is only partially true. Figure~\ref{XX} shows the cumulative distribution of the variance of cost matrix elements for sixty windows. It shows that though the the workload does not change much over time, the variance of cost matrix elements is quite high. Figure~\ref{XX} shows the relationship between variance and the memory footprint of cost matrix elements. It demonstrates that the high variance is not dominated by operators with low memory footprint. Instead, we observe high variance for operators with high memory footprint as well. 

\paragraph{Cost of not adapting over time.}
Now that we understand that Sonata's assumption about workload dynamics do not hold in real-world settings, we now quantify the impact of not adapting the query plans over time. To illustrate this point, we select a pair of consecutive windows. We use Sonata to compute the query plans for the two windows. We then apply both these plans for the second window and measure the load at the stream processor. The difference in load for the two plans quantifies the cost of not adapting, i.e., using a stale query plane. Figure~\ref{XX} shows the cumulative distribution of increase in load at the stream processor for all sixty window pairs in dataset~1. It shows that using the query plan computed for the last window itself can result in XX \% increase in load at the stream processor. 

When we use a stale query plans, there are three possibilities, i.e., the amount of memory required to execute a stateful operator in the data plane is (1)~exactly the same, (2)~less than, and (3)~more than what was assigned in the previous window. Given the dynamic nature of cost matrices, the first case is highly unlikely. The second case results in under-utilization of limited switch memory and entails an opportunity cost. In the third case, Sonata sends all the packets from this operator onwards to the stream processor (for cases where a query has more than one stateful operator). As a result, such under provisioning not only sends more packets to the stream processor, it also leaves some of the operators unused (more opportunity cost). 

\ag{Next two paragraphs are not adding a lot of value.}
Figure~\ref{XX} shows how the increase in workload is related to changes in the cost matrices. In this graph, each data point is a tuple of normalized difference between the two cost matrices and increase in load at the stream processor. This graph shows that even when the difference between the two cost matrices is smaller, the cost of using stale plans is higher---indicating the over sensitive nature of Sonata's query plans to smaller changes in workload. 

To quantify the impact of not adapting query plans over longer horizons, we used Sonata's query planner to compute query plans for all sixty windows in dataset~1. We then applied the plan selected for a window for all other fifty nine windows. Figure~\ref{XX} shows the cost of not adapting query plans over longer horizons. Compared to one-window horizon (Figure~\ref{XX}), the increase in load at stream processor is XX \% higher. Here. note that the higher end of the load in this distribution is of the same order as load at stream processor without hardware switches. These results illustrate that inability to adapt query plans over time offsets the scalability promises offered by hardware switches. 






% We need to answer the following questions here: 
% \begin{itemize}
%     \item What is changing over time? How are changes in workload related to changes in cost matrices over time? Takeaway: the total workload is not changing much, but cost matrices have a high variance. Even operators with high memory footprint vary a lot
%     \item What's cost of not adapting query plans? Takeaway: using stale plans contribute to significant increase in load at the stream processor.
%     \item Diagnose the root cause of such a steep rise in load at stream processor over time. Takeaway: register sizing and register sizes are too sensitive to changes. 
% \end{itemize}



% \paragraph{Deep-dive with an example}

\subsection{Possible Approaches}
These observation motivates a solution that can better handle workload dynamics and help reduce the load at the stream processor. At a higher level, the two ends of the design spectrum are: (1)~{\em static query planning}: where the query planner uses the input cost matrices more effectively to compute a static query plan that works well for longer time horizons, i.e., tens of future windows; (2)~{\em dynamic query planning}: where the query planner dynamically updates the query plans at shorter time scales (order of 1-2 windows) while satisfying all the constraints related to dynamically reconfigure the packet processing pipeline at runtime. 

\subsubsection{Static Query Planning}
From the operational complexity perspective, static query planning is highly desired at it avoids making any reconfiguration to the packet processing pipeline at runtime.

\paragraph{Static query-planning approaches.}
 Currently, Sonata takes to median value of all the input cost matrices to compute a query plan. One approach can be to extend Sonata's query-planning ILP to optimize for all the input windows. For such an ILP, the number of constraints increases linearly with the number of input windows. Given the computational complexity of solving the ILP for a single window, we expect this ILP to taker orders of magnitude more time to converge to a (near-)optimal solution. Moreover, such a query plan is overfitted for the input cost matrices, and suffers from similar problems as Sonata in handling the dynamics of future windows. 

Another approach can be to focus on improving the input, i.e., the cost matrix, to Sonata's query planning ILP. Intuitively, if the cost matrix input to the ILP can capture the dynamics of future windows more effectively, then it can possibly handle traffic dynamics more effectively. We explored multiple heuristic-based approaches on how to determine the best input cost matrix such that it can handle traffic dynamics more effectively. For brevity reasons, we have presented the details of different heuristics we developed for static query planning in Appendix~\ref{XX}. The takeaway from these explorations is that these approaches do perform better than Sonata, but still leave a lot of scope for improvement. We present the comparisons between static and dynamic query planning in Section~\ref{XX}. 

\paragraph{Why static query planning is ineffective?}
The efficacy of static query planning approaches depend on how well they can predict the dynamics for future windows over longer time horizons, which is fundamentally challenging. Inability to capture these future trends result in solutions that are ineffective for scenarios where network resources are scarce. More concretely, given the future uncertainties, one approach is to overprovision the input cost matrix such that we double the memory requirements for all the cost matrix elements, and then use this new cost matrix to compute the query plan. Such an approach will work well for operators whose memory requirements are higher than the median value in the future, but for most cases it results in wasteful memory allocation of limited switch memory, resulting in higher load at the stream processor for most windows (see Figure~\ref{XX}).  

\subsubsection{Dynamic Query Planning}
Dynamic query planning has the capability to identifying changes in memory requirements for different cost matrix elements (or operators) at shorter time scales, and explore a query plan that can make more effective usage of limited switch resources. 

One naive approach can be to use Sonata's query planner to compute query plans for every window. Though, such an approach can help reduce the load at stream processor (see Figure~\ref{XX}), it is impractical. First, it requires changing the refinement plan and register sizes at runtime. Changing refinement plan at runtime affects query's accuracy and changing register sizes at runtime require recompiling the data-plane target, which can take the switch down for few seconds---disruptive. Second, it requires solving the ILP for an NP-hard problem. Solving this ILP to get (near-)optimal solution takes hundreds of seconds, and is thus, not suited for real-time decision making. Finally, to compute the query plans this approach requires the cost matrix for that window as input, which is not possible. 

\paragraph{How can we make dynamic query planning practical?}
Given these limitations, the question is whether it is possible to design a dynamic query-planning solution that can handle the workload dynamic in a more practical manner. In this paper, we show that it is possible to develop such a solution. More concretely, we show that it is possible to compute refinement plans and register sizes such that they make dynamic mapping of operators to hash-tables more effective at runtime. Here, we demonstrate that such bootstrapping is less dependent on workload dynamics and more on the structure of input queries---invariant over time. 

To compute these dynamic mapping we only require predicting the workload for a single window horizon, that too for a subset of cost matrix elements (as the refinement plan is fixed). Unlike static query planning where to get better results, one needs to accurately predict all elements for all future cost matrices, predicting the requirements for subset of cost matrix elements for a single window is more tractable. Moreover, we observed that the cost matrices have a low rank, i.e., different cost matrix elements exhibit high correlation, which further simplifies the learning model. 

Finally, given that at runtime, the query planner only needs to decide how to map operators to hash tables, the problem is much simpler than solving the full query planning ILP. Though, the ILP to solve this problem still takes few hundreds of second to compute the optimal mapping, we developed a greedy heuristic that only took few tens of millisecond to find (near-)optimal mappings. 


% More concretely, given that changing refinement plans and register sizes at runtime is not practical, then we can only change the mapping of operator to hash-table mapping. We show that it is possible to compute the refinement plan and register sizes using limited input data such that the dynamically remapping of operators to hash table in the data plane can significantly reduce the load at the stream processor. We also show that it is possible to train an LSTM-based model to predict the future 
% We now discuss how we can address each of the challenges discussed above to make dynamic query planning more practical. First, 

% \paragraph{Takeaways.}


% \begin{itemize}
%     \item Two ends of the spectrum: (1)~static query planning: compute one static plan that works for multiple windows in the future, (2)~dynamic query planning: compute plans that work for 1-2 windows at a time.
%     \item Static query planning: 
%     \item Dynamic query planning: 
%     \item Dynamic makes sense 
% \end{itemize}

% \paragraph{Optimal $\rightarrow$ Impractical}
% Highlight practical limitations
% \begin{itemize}
%     \item refinement plans
%     \item register sizes
% \end{itemize}

% \paragraph{Results preview.}
% Present the CDF with stale, optimal, and \system's performance.


% Sonata assumes that the median cost matrices of the training data (a handful of windows) are representative of future workload, and the query plans will continue reducing the workload at the stream processor. Figure~\ref{XX} shows the cost of using stale plans. \ag{TODO: add the stale plan cost result here.}. To handle traffic dynamics, it keeps track of hash collisions in the data plane. It argues that if the collision rate exceeds a pre-determined threshold, it will recollect the packet traces and recompute the cost matrices to find a new query plan. Such an approach has multiple issues, which affect Sonata's deployability. First, collecting raw packet traces is an expensive task and cannot be performed frequently. Second, computing cost matrices requires executing all possible variants of the input query over the raw packet traces. For example, it takes XX seconds for the BigQuery-based program to compute the cost matrix for XX three-second windows. Performing such an operation locally (avoid sending raw packet traces to the cloud) is not only prohibitively expensive but is also too slow for updating the query plans in a timely manner. Third, naively recomputing the query plan will entail resizing the hash tables in the data plane and will thus require reconfiguring the data plane. Reconfiguring the switch at runtime requires draining (and un-draining) the switch, which is impractical for most operational scenarios. 

==> design-roadmap.tex <==


\section{Dynamic Query Planning in a Nutshell}
\label{sec:dynamiq-design}
%\rjh{Proposed re-sectioning. New signpost paragraph needed here -- punting for now until we get consensus on this restructure.}

In this section, we describe our approach to developing dynamic query plans that can be practically implemented and boost the scalability of modern hybrid data-plane/host-based network streaming analytics systems. We first describe the challenges in developing dynamic query plans.  We then describe our approach that consists of a one-time boot-strapping effort at start time to decide on an initial query plan (Section~\ref{ssec:bootstrap}) and leverages dynamic operator mapping at runtime (Section~\ref{ssec:dynamop}). These two key components are described in more detail in Sections 4 and 5 below.

\subsection{Challenges to Planning Dynamically}

In practice, static query plans are highly desirable because they avoid the need to reconfigure the data plane packet processing pipeline at runtime. With a few exceptions, performing such configuration changes is not possible at runtime and requires taking the data plane target offline for a short period of time (typically XX msec) which can be unacceptable in real-world production settings. For example, reconfiguring register sizes requires taking the switch offline. Also, while it is possible to change a refinement plan at runtime, it is highly problematic and ill-advised because it affects the queries' accuracy in ways that are difficult to quantify. \rjh{Have we solved this problem in the general case?  Isn't dynamic query planning only going to exacerbate this issue?}

However, as the Sonata example shows, even relying on diligently-chosen, but stale, static query plans can result in situations where almost the entire input workload ends up being processed in user space.  This wastes data plane resources and begs the question of why bother offloading processing to the data plane at all.  At the same time, the opportunity costs we identified earlier in Section~\ref{ssec:static-harmful} hint that dynamic query plans could be both efficient (\ie can effectively leverage the scarce data plane resources by adapting to time-varying operator memory requirements at runtime) and practical (\ie can be computed online and implemented at runtime without any oracular knowledge of the future workload).

%\paragraph{A straw man proposal for a dynamic query plan.} One naive approach to move beyond Sonata's static query plan is to use its ILP solver to compute a query plan for each and every window. Although this approach is theoretically feasible and can help reduce the load at the stream processor (see Figure??), it is highly impractical. First, it requires changing the refinement plan and register sizes at runtime. However, changing the refinement plan at runtime affects a query’s accuracy, and changing register sizes at runtime requires recompiling the data-plane target which is in general disruptive because it requires taking the switch offline for a few seconds.  Second, it requires solving an NP-hard problem for each window, and Sonata's ILP solver is already not suited for (close-to) real-time decision making because it takes hundreds of seconds to compute a (near-)optimal solution. Finally, to compute the query plan for a given window, this approach requires the cost matrix for that window as input which is not available in real time.

%\paragraph{On making dynamic query planning practical.} Realizing that static query plans can largely be ruled out as efficient and effective solutions to the problem faced by today's hybrid network streaming data analytics systems begs the question whether the answer lies in dynamic query planning. In particular, we are interested in knowing whether dynamic query plans can be more effective than their static counterparts in efficiently utilizing limited data plane resources by recognizing and adapting to changes in memory requirements for different operators (\ie cost matrix elements) in a more agile fashion; that is, at time scales that allow for the data plane execution of the proper responses to the observed changes. 

%A main lesson learned from the Sonata example for architecting modern hybrid data-plane/host-based network streaming analytics systems more generally is that while iterative refinement helps greatly with scaling query execution in the data plane (originally shown in~\cite{sonata-sigcomm}), it negatively impacts the effectiveness of static query plans to the point where they render the overall system largely futile by making highly inefficient use of the available data plane resources. In this section, we provide a road-map for our approach to developing dynamic query plans that retain the scalability benefits of iterative refinement and are at the same time agile (\ie can adapt to operator memory requirements that vary over time), efficient (\ie can effectively leverage the scarce data plane resources), and practical (\ie can be implemented at runtime). Our approach to dynamic query planning leverages dynamic operator mapping at runtime and consists of a one-time bootstrapping effort at start time to decide on an initial query plan. These two ingredients are described in more detail in Sections 4 and 5 below.

\subsection{Bootstrapping an Initial Query Plan}
\label{ssec:bootstrap}

\paragraph{Problem: Changing refinement plan and register sizes at runtime is impractical.} Before addressing how to best map operators to data plane hash tables, we must first select an initial refinement plan and register size configuration that are ``future-proof", i.e., a configuration that exploits structure in the input queries and can adapt to the dynamics of the input workload without recompiling the data plane pipeline. Choosing the wrong plan could result in high workload for the stream processor and choosing the wrong register size configuration could leave insufficient resources for dynamically mapping operators to hash tables. However, combining the right initial query plan with dynamic operator to hash-table mapping, allows us to adapt to traffic dynamics in the future and ensure that the workload (\ie number of tuples) sent to the stream processor is as small as possible. 

\paragraph{Partial Solution: Total Operator Memory Heuristic.} We address the problem of selecting an initial query plan by developing a heuristic solution that exploits structure within the input queries and is largely robust to varying input workloads. For computing the initial refinement plan, we leverage our intuition that for the purpose of dynamically mapping operators to hash-tables at runtime, it is more effective to have fewer operators and smaller overall or total operator memory (TOM). The resulting ``TOM-heuristic" selects an initial refinement plan that has the lowest TOM as well as the least number of stateful operators. In section, we show that this heuristic works well for determining the initial refinement plans, and that refinement plans with high TOM fail to minimize the workload on the stream processor. 

\paragraph{Partial Solution: ``Slice-n-replicate'' Heuristic.} Given an initial refinement plan, the problem of register sizing can again be modeled as an ILP. Unlike the ILP for the static case, however, the resulting ILP is both computationally intractable and over-fitted for the input data. Solving this ILP is further complicated by special sizing constraints in the data plane that impose upper bounds on memory that can be allocated to individual hash-tables as well as to all the hash-tables in a physical stage.  To solve this problem, we develop a heuristic that leverages the intuition that a register size configuration with more hash-tables and more diversity in hash-table sizes is preferable when it comes to efficiently mapping operators to hash-tables at runtime. We show that the resulting ``slice-n-replicate" heuristic (SnR-heuristic, for short) efficiently uses available data plane memory and works well in conjunction with our operator mapping heuristic in adapting to variations in the input workload. 

%The bootstrapping effort concerns the computation of both a refinement plan and an allocation of register sizes such that together, they facilitate the dynamic mapping of operators to hash-table at runtime and ensure that the mapping is effective. In the process, we demonstrate that such bootstrapping is less dependent on the network traffic workload dynamics and more on the structure of input queries which we assume in this paper to be invariant over time.

\subsection{Dynamic Operator Mapping at Runtime}
\label{ssec:dynamop}

\paragraph{Problem: Computing the optimal operator to hash-table mappings is NP-hard and requires oracular knowledge of the future workload.} For a given refinement plan and a given register size configuration, the problem of finding a (near-) optimal mapping of operators to  hash-table sizes for future windows such that the mappings minimize the load at the stream processor can be modeled as an ILP. However, similar to the ILPs discussed previously, solving this particular ILP is also intractable, especially for making mapping decisions at runtime. Solving this ILP is further complicated by additional constraints that specify how operators can be mapped to hash-tables (and vice versa) and what ordering relationships need to be enforced for queries that consist of multiple stateful operators. Finally, any practical approach could only use historical workload information and could not practically know the future workload.

\paragraph{Partial Solution: Greedily Mapping Operators.} We solve this problem by developing an algorithm that respects the various constraints yet is still tractable and effective. We first reduce the ILP to a constrained non-standard Knapsack problem and then develop a greedy heuristic that differs from the various approximation schemes that have been developed for Knapsack-like problems in the literature and relies on domain knowledge instead. 

\paragraph{Solution (part II): Using a prediction model instead of oracular knowledge to deal with future workload.} {\em TDB once the prediction model is in place.}

==> interface.tex <==
\section{Unified Query Interface}
\label{sec:prog-abs}

This section presents \system's query interface and shows example queries to
illustrate the types of queries that existing systems can and cannot support. 
\system provides a query interface that is as expressive as modern stream
processors but opportunistically achieves the scalability of data-plane execution.
Although \system uses programmable switches to scale query execution, the 
expressiveness of its query interface does not depend on the computational 
capabilities of these switches. 
\system's stream processor simply executes the operations for which no more data-plane resources are 
available or which are not supported by the switch (\eg, payload processing or 
floating-point arithmetic).
%It executes all the operations that are not supported 
%in the switch, such as ones requiring payload processing or floating-point operations, 
%in the stream processor.

\subsection{Dataflow Queries on Tuples}
\smartparagraph{Extensible tuple abstraction.} Information in packet headers
naturally constitute key-value tuples (\eg, source and destination IP address,
and other header values). This structure lends itself to a tuple-based
abstraction~\cite{sonata-hotnets}. Of course, an operator may want to write
queries based on information that is not in the IP packet header, such as the
application protocol, or DNS query type. To facilitate a broader range of queries, 
\system allows an operator to extend the tuple interface to include other fields 
that could be extracted by either the programmable switch or the stream processor. 
For example, they can specify customized packet-parsing operations for 
programmable switches in a language such as P4. Based on such a
specification, the parser can extract all portions of the packet that pertain to
the query. \system parses tuples on the switch whenever possible, shunting
packets to the stream processor only when the query requires sophisticated
parsing (\eg, parsing of the packet's payload) or join operations that the switch 
itself cannot support.
%information that requires a join with auxiliary information such as a routing table.

\ifx \TR \undefined
\smartparagraph{Expressive dataflow operators.} Many network telemetry tasks
require computing aggregate  statistics over a subset of traffic and joining
the results from multiple queries, which can be expressed as a sequential
composition of dataflow operators (\eg, filter, map, reduce).
Gigascope~\cite{gigascope},  Chimera~\cite{chimera}, and Marple~\cite{marple}
all use such a programming model, which is both familiar and amenable for
compilation to programmable switches~\cite{marple}. Section~
\ref{sec:pisa-dataflow} describes how \system compiles queries across the stream
processor and switch. We include an overview of all the operators \system
suports in an extended technical report~\cite{sonata-tech-report}. Stateful
dataflow operators are all executed with respect to a query-defined time
interval, or window. For example, applying {\tt reduce} over a sum operation
will return a result at the end of each window. Each query can explicitly
specify the interval's duration for stateful operations.
\else
\smartparagraph{Expressive dataflow operators.} Many network telemetry queries
require computing aggregate  statistics over a subset of traffic and joining
the results from multiple queries, which can be expressed as a sequential
composition of dataflow operators (\eg, filter, map, reduce).
Gigascope~\cite{gigascope},  Chimera~\cite{chimera}, and Marple~\cite{marple}
all use such a programming model, which is both familiar and amenable for
compilation to programmable switches~\cite{marple}. Section~
\ref{sec:pisa-dataflow} describes how \system compiles queries across the stream
processor and switch. Table~\ref{tab:interface} summarizes \system's dataflow 
operators. Stateful dataflow operators are all executed with respect to a query-defined 
time interval, or window. For example, applying {\tt reduce} over a sum operation
will return a result at the end of each window. Each query can explicitly
specify the interval's duration for stateful operations.

%Here, stateless operators, such as {\tt filter} and {\tt map} emit results immediately
%after operating on an input tuple. Stateful operators such as {\tt reduce}, {\tt
%distinct}, and {\tt join} emit results at the end of a query-defined time window
%of $W$ seconds.  

\begin{table}[h!]
\begin{footnotesize}
\centering
\resizebox{.85\linewidth}{!}{%
\begin{tabular} {| l m{2.0in} |}
\hline
{\bf Operator} & {\bf Description} \\ \hline
{filter}($p$) & Filter packets that satisfy predicate $p$.\\
{map}($f$)  & Transform each tuple with function $f$.\\
{distinct()}  & Emit tuples with unique combinations of fields.\\
{reduce}($k$, $f$) & Emit result of function $f$ applied on key $k$ over the
input stream.\\ 
{join}($k$, $q$) & Join the output of query $q$ on key field $k$ \\
\hline
\end{tabular}
}
\end{footnotesize}
\caption{\system{}'s Dataflow Operators.  All stateful operators execute with
respect to a window interval of $W$ seconds.}
\label{tab:interface} 
\end{table}
\fi

\smartparagraph{Limitations.} \system supports queries operating at packet-level
granularity, as in existing declarative telemetry systems~\cite{gigascope,
chimera,opensoc,marple}; it cannot support queries that require reassembling 
a byte stream, as in Bro~\cite{bro}. \system also currently compiles each query to a 
single switch, {\em not} across multiple switches.  
We leave compiling arbitrary queries to multiple switches as future work, but the
set of single-switch queries considered in this paper is nonetheless directly 
applicable to real-world deployments such as a border switch or an 
Internet exchange point (IXP).
%The set of single-switch 
%queries we present are still practical for many deployments, such as on a 
%border switch or at an Internet exchange point (IXP).  We leave 
%compiling arbitrary queries to multiple switches as future work.

\subsection{Example Network Telemetry Queries}
\label{ssec:queries}

We now present three example queries: one that executes entirely in the data
plane, a second that involves a join of two sub-queries, and a third that
requires parsing packet payloads. Table~\ref{tab:apps} summarizes the 
queries that we have implemented and released publicly along with the 
\system software~\cite{sonataqueries}.

\begin{figure}[t!]
\begin{lstlisting}[language=query2,basicstyle=\footnotesize, 
basicstyle=\footnotesize, numbers=left,xleftmargin=2em,frame=single,
framexleftmargin=2.0em, captionpos=b, label=tcp-conn, 
caption=Detect Newly Opened TCP Connections.]
packetStream(W)
.filter(p => p.tcp.flags == 2)
.map(p => (p.dIP, 1))
.reduce(keys=(dIP,), f=sum)
.filter((dIP, count) => count > Th)
\end{lstlisting}
\ifx \compress \undefined
\else
\vspace*{-1\baselineskip}
\fi
\end{figure}

\smartparagraph{Computing aggregate statistics over a subset of traffic.} 
Suppose that an operator wants to detect hosts that have too many 
recently opened TCP connections, as in a SYN flood attack.
Detection requires parsing each packet's TCP flags and destination 
IP address, as well as computing a sum over the destination IP address 
field. Query~\ref{tcp-conn} 
first applies a {\tt filter} operation (line 2) over the entire packet stream
to select TCP packets with just the {\tt SYN} flag set. It then counts the
number of packets it observed for each host (lines 3--4) and reports the hosts
for which this count exceeds threshold {\tt Th} at the end of the window (line
5). This query can be executed entirely on the switch, so existing systems (\eg,
Marple~\cite{marple}) can also execute this type of query at scale.
%Existing telemetry systems, such as Marple~\cite{marple} 
%that performs computation only in the data plane, can easily support and 
%scale this type of simple query.


\smartparagraph{Joining the results of two queries.} A more complex query
involves joining the results from two sub-queries. To detect a Slowloris
attack~\cite{slowloris}, a network operator must identify hosts which use many
TCP connections, each with  low traffic volume. This query 
(Query~\ref{slowloris}) consists of two sub-queries: the first sub-query counts the number
of unique connections by applying a  {\tt distinct}, followed by a {\tt reduce}
(lines~1--6).  The second sub-query counts the total bytes transferred for each host
(lines~8--11). The query then joins the two results (line 7) to compute  the
average connections per byte (line 12) and reports hosts whose average number
of connections per byte exceeds a threshold {\tt Th2} (line~13). 
Marple~\cite{marple} cannot support this query as it applies a join after an 
aggregation operation (reduce). Also, this query cannot be executed entirely 
in the data plane as computing an average requires performing a division 
operation. Even state-of-the-art programmable switches (\eg, Barefoot 
Tofino~\cite{tofino}) do not support the division operation in the data plane. 
In general, existing approaches that only use the data plane for query execution 
cannot support queries that require complex operations that cannot be executed 
in the switch. In contrast, \system's query planner partitions the query for partial 
execution on the switch and performs more complex computations at the stream 
processor.

%Marple~\cite{marple} cannot support this query as it applies a join operation after an 
%aggregation operation (reduce). Additionally, the query involves computing an average, which requires performing division;
%even state-of-the-art programmable switches do not support this operation in
%the data plane~\cite{tofino}. Some queries will naturally need to perform operations 
%that are more sophisticated than the switch can support; in such cases, existing
%approaches cannot execute these kinds of queries at all. In contrast,
%\system's query planner can partition the query for partial execution on the
%switch and perform more sophisticated computation not available in the
%switch at stream processor.

Although this query is written to detect hosts for which the average bytes per
connection exceeds a threshold, it is equivalent to detecting hosts for which
the average bytes per connection is {\em less than} a different threshold;
%in Section~\ref{sec:qref}, 
%we discuss why it is desirable to express the query as the former instead of the latter.
we explain in Section~\ref{sec:qref} why it is desirable to express this query using a 
``greater than'' instead of a ``less than'' condition.


\begin{figure}[t!]
\begin{lstlisting}[language=query2,basicstyle=\footnotesize, 
basicstyle=\footnotesize, numbers=left,xleftmargin=2em,frame=single,
framexleftmargin=2.0em, captionpos=b, caption=Detect Slowloris Attacks., label=slowloris]
packetStream
.filter(p => p.proto == TCP)
.map(p => (p.dIP,p.sIP,p.tcp.sPort))
.distinct()
.map((dIP,sIP,sPort) =>(dIP,1))
.reduce(keys=(dIP,), f=sum)
.join(keys=(dIP,), packetStream
  .filter(p => p.proto == TCP)
  .map(p => (p.dIP,p.pktlen))
  .reduce(keys=(dIP,), f=sum)
  .filter((dIP, bytes) => bytes > Th1) )
.map((dIP,(byte,con)) => (dIP,(con/byte))
.filter((dIP, con/byte) => (con/byte > Th2)
\end{lstlisting}
\ifx \compress \undefined
\else
\vspace*{-1\baselineskip}
\fi
\end{figure} 

\begin{figure}[t]
\begin{lstlisting}[language=query2,basicstyle=\footnotesize, 
basicstyle=\footnotesize, numbers=left,xleftmargin=2em,frame=single,
framexleftmargin=2.0em, captionpos=b, caption=Detect Zorro Attacks., label=zorro]
packetStream
.filter(p => p.tcp.dPort == 23)
.join(keys=(dIP,), packetStream
  .filter(p => p.tcp.dPort == 23)
  .map(p => ((p.dIP,p.nBytes/N), 1))
  .reduce(keys=(dIP, nBytes), f=sum)
  .filter(((dIP,nBytes),cnt1) => cnt1 > Th1))
.filter(p => p.payload.contains('zorro'))
.map(p => (p.dIP,1))
.reduce(keys=(dIP,), f=sum)
.filter((dIP, count2) => count2 > Th2)
\end{lstlisting}
\ifx \compress \undefined
\else
\vspace*{-1\baselineskip}
\fi
\end{figure}

\smartparagraph{Processing packet payloads.}
Consider the problem of detecting the spread of malware via
telnet~\cite{iotpot}, which is a common tactic targeting IoT
devices~\cite{mirai_operations}. Here, miscreants use brute force to gain
shell access to vulnerable Internet-connected devices. Upon successful login,
they issue a sequence of shell commands, one of which contains the
keyword ``zorro.'' The query to detect these attacks first looks 
for hosts that receive many similar-sized telnet packets followed by a telnet 
packet with a payload containing the keyword ``zorro.'' The query for this 
task has two sub-queries (Query~\ref{zorro}): the first part identifies hosts 
that receive more than {\tt Th1} similar-sized telnet packets rounded off by 
a factor of {\tt N} (lines 4--7). The second part joins (line 3) the output of the 
first sub-query with the other and reports hosts that receive more than {\tt Th2} 
packets and contain the keyword ``zorro'' in the payload (lines 8--11). Since
this query requires parsing packet payloads, many existing approaches cannot
support it. In contrast, \system can support and scale these queries by
performing as much computation as possible on the switch and then performing the
rest at the stream processor.




%division operations in the 
%data plane is costly, even for modern switch chipsets; as a case in 
%point, even the state-of-the-art Tofino~\cite{tofino} switch does not 
%support division operations in the data plane. Thus, existing 
%data-plane only telemetry systems including Marple~\cite{marple} 
%cannot support such queries. 

%This query involves
%combining several separate counts across the packets and
%also requires processing the packet’s payload.
%This query also has two sub-queries.

%\smartparagraph{Expressiveness.} 

%It not only requires where to place each
%dataflow operatorDetermining how to place dataflow
%operators and It requires 
%
%query over 
%Extending \system to support network-wide telemetry queries is non-trivial. requires reasoning about how to determine threshold 
%All of the queries
%currently run only on a single programmable switch. 
%Supporting distributed data-plane targets and incorporating packet history---both
%within a byte stream and on a path---are excellent avenues for follow-up work.

%\system{}'s query interface allows it to abstract the details 
%of {\em where} each query operator runs and {\em how} the underlying targets 
%perform those operations. \system's query planner decides how and where to 
%execute the input queries allowing identical queries to execute over different 
%choices of streaming or data plane targets without modification. This feature 
%ensures that the telemetry system is flexible and easy to maintain.



%\system's query interface is based on dataflow frameworks. 


%query interface takes advantage of the inherent similarity between
%data plane and dataflow processing paradigms and presents a single
%interface for expressing complex queries. These queries are based on an
%extensible packet-as-tuple abstraction and execute both in the data plane and
%at a stream processor. We introduce this interface and show how applying
%dataflow operators over tuples can support a wide range of network telemetry
%applications.  We then show how to compile queries expressed as a composition of
%data flow operators to a sequence of match-action tables in the data plane.


  
%\subsection{Unifying Dataflow and the Data Plane}
%\label{ssec:dataplaneflow}
%
%The processing model for modern PISA
%targets aligns well with the processing model for streaming analytics platforms,
%such as Spark Streaming~\cite{dstream}.  The processing pipelines for both can
%be represented by a directed, acyclic graph (DAG) in which each node of the
%graph performs some computation on an incoming stream of structured data.  For
%stream processors, the nodes in the DAG are dataflow operators and the
%structured-data stream consists of tuples.  For PISA targets, the nodes in the
%DAG are match-action tables and the structured-data stream consists of packets.
%Given this inherent symmetry, an ordered set of dataflow query operators could
%map to an ordered set of match-action tables in the data plane.  Similarly, by
%transforming packets into named-tuples, a general purpose stream processor could
%perform any packet processing that is expressible using that platform.  By
%choosing to express queries as a composition of dataflow operators, \system
%allows network operators to write a single query that can be flexibly executed
%on both modern data plane targets and stream processors.  \system, therefore,
%makes use of both the rich computation available at the stream processor and the
%high-speed processing available in the data plane.  Sonata's query planner now
%has the option of choosing whether a given query will be executed in the data
%plane or at the stream processor; we later discuss this decision procedure in 
%Section~\ref{ssec:qplan_problem}.

%\subsubsection{Extensible Packet Tuple Abstraction}
%\label{ssec:prog-abs}
%%%%
%%%% Packet tuple
%%%%
%Packets carry not only information in their header fields and payload, but also
%the meta information about the state of the underlying network, such as the
%time when a packet arrives at a switch or number of hops it traversed in the
%network. \system{} provides an intuitive interface for expressing queries over
%the superset of fields extracted either in the data plane or in user space. This 
%abstraction is inherently flexible because the list of fields in the packet tuples
%can incorporate new header and metadata fields as the underlying data plane
%evolves, for example, reading the sizes of queues the packet experienced en
%route~\cite{int}.
%
%
%%To extend the packet tuple with query-specific fields, 
%\system has an extensible parser that unifies the parsing capabilities of the
%available data plane and streaming targets. The parser extracts from the raw
%packets all fields required to satisfy the set of input queries.
%\system seeks to perform parsing in the data plane whenever possible
%and directs packets to the stream processor for parsing only when necessary. In
%user space, \system employs extensible, user-defined parsing modules that
%extract fields for many standard protocols. For example, for the case
%of the Zorro attack query, it parses all of the packet fields in the data plane
%except the {\tt payload} field which is parsed in user space.
%
%\subsubsection{Expressive Dataflow Operators}
%\label{ssec:dataflow}
%Network telemetry applications often require computing aggregate statistics over 
%a subset of traffic and joining the results from multiple queries. Most of these tasks 
%can be expressed using declarative queries that compose dataflow operators.
%\system{}'s query interface allows it to abstract the details of {\em where} 
%each query operator runs and {\em how} the underlying targets perform those 
%operations. \system's query planner decides how and where to execute the input
%queries allowing identical queries to execute over different choices of
%streaming or data plane targets without modification. 
%This feature ensures that the telemetry system is flexible and easy to maintain.
%
%
%
%%\system's query interface is based on dataflow frameworks. 
%Table~\ref{tab:interface} describes the operators that \system supports.
%Stateless operators, such as {\tt filter} and {\tt map} emit results immediately
%after operating on an input tuple. Stateful operators such as {\tt reduce}, {\tt
%distinct}, and {\tt join} emit results at the end of a query-defined time window
%of $W$ seconds.  \system also supports the {\tt join} operator
%over consecutive window intervals. This feature provides additional flexibility for 
%network operators to employ a query only after observing an event of interest.
%For example, in Query~\ref{zorro}, it makes sense to look for the keyword ``zorro" 
%in the payload after the attacker has attempted to gain shell access by sending 
%excessive similar-sized telnet packets. 
%
%\rjh{Enrich the discussion of join}subsection{Example \system{} Queries}
%Network operators can express various queries
%using the interface described above. 



%\mcnote{Is this the right place to discuss this? Here could highlight instead that for simplicity we reason about a single switch. Later we discuss the issue of how to extend to multiple switches (which is left to future work but we should have ideas of what to do).}




==> intro-vers2.tex <==
\section{Introduction}
\label{sec:intro}


\begin{figure}[t] 
\begin{center}
\includegraphics[scale=0.6]{figures/dynamiq}
\caption{\system's architecture for dynamic query planning and execution.}
\label{fig:sonata-dynamiq}
\vspace{-.25in}
\end{center}
\end{figure}

Networks supporting Internet-connected applications and devices have witnessed exponential growth in both scale and complexity. To effectively manage these networks, operators must keep track of coarse- to a very fine-grained application- or service-specific aspects of the traffic to detect (and ultimately react to) an increasingly diverse set of performance- or security-related network events in (near) real-time. Unfortunately, humans can no longer perform many of these tasks.  To automate these tasks, today’s networks rely increasingly on modern network streaming analytics systems capable of running a large number and wide range of different queries at line rate for up to billions of packets per second. 
\ag{We should not call out systems like Flowradar and BeauCoup here as it backfired for us in the past. In the iteration, we will offer comparisons with Marple, UnivMon, etc.}
A common feature of many of these systems (\eg Sonata~\cite{sonata}, Marple~\cite{marple}, Flowradar~\cite{flowradar}, BeauCoup~\cite{beaucoup}) is that they offload a portion of query execution to programmable data-plane targets (\eg Barefoot Tofino~\cite{tofino}) that send intermediate results to state-of-the-art stream processors (\eg Apache Flink~\cite{flink}) for further back-end processing. However, since today’s programmable data planes are inelastic by design and, in general, highly constrained by limited hardware resources (\eg memory, CPU), a critical function of many of these systems is {\em query planning}.  Each system must specify precisely how to configure the packet-processing pipelines in the data plane to support the various dataflow operators for a given set of queries while also accounting for the dynamic nature of real-world network traffic workloads. In practice, query planning comes down to uncovering structural properties of the given queries and learning about patterns in the arriving traffic workload so as to make the best use of the available hardware resources in the programmable data plane. In fact, the deployability of some of these promising hybrid network streaming analytics systems hinges largely on the scalability gains that result from carefully designed query plans that can be implemented in practice and attempt to maximize query execution upfront (\ie in the data plane) and minimize the workload sent to the back end (\eg stream processor).

While query planning can result in static or dynamic query plans, existing hardware-based network streaming analytics systems are generally concerned with strictly static plans, mainly because of their tractability and simplicity. A key feature of static query plans is that they are ``early-binding" in nature, i.e., they make low-level decisions such as configuring the packet processing pipeline at compile time itself. The upside of this ``early binding" is that the runtime complexities are minimal, but the downside is that it prevents these systems to react to changes in the queries' input workload over time. 

% To better understand this tradeoff, we consider Sonata~\cite{sonata}, which uses static query plans. To scale query execution, Sonata not only partitions the input queries between the switch and stream processor, but it also refines the input queries over consecutive windows, enabling it to selectively spend resources on portions of traffic relevant to the input queries. Sonata's query planning decisions can be divided into three parts: (1)~\textit{refinement plan}: how to iteratively refine each query, (2)~\textit{register sizing}: how to configure register sizes for stateful operators, and (3)~\textit{operator mappings}: how to map dataflow operators to stateful/stateless data structures in the data plane. 

% To compute query plans, Sonata takes a sample of packet traces as input and uses an integer linear program (ILP) solver to determine a static query plan. This plan minimizes the stream processor's load and assumes that future traffic is similar to the one used as input. However, we observe that, in practice, such an assumption does not hold. As a result, the usage of static query plans increases the amount of traffic sent to the stream processor by 3-4 orders of magnitude, which is of the same order as the stream processor's load without any query partitioning.

% While query planning can result in static or dynamic query plans, existing hardware-based network streaming analytics systems that touch on query planning in one form or another are in general only concerned with strictly static plans, mainly because of their tractability and simplicity. A key feature of static query plans is that they are ``early-binding" in nature, meaning that low-level decisions such as which dataflow operators use how many ALUs at which physical stages are only made at compile time and cannot be changed at runtime. This inability to react to changes in the queries' input workloads makes static query plans ill-suited for benefiting from the unique opportunities afforded by programmable data plane targets and can cause such the system as a whole to exhibit such poor performance that its deployability in practice is in doubt. 

Motivated by these observations, we explore in this paper dynamic query planning. Specifically, we focus on developing query-planning algorithms that are both performant and practical; that is, can adapt to changes in the input workload while ensuring that the runtime overheads are minimal. We integrate these algorithms into a production-ready network streaming analytics system. To this end, we present the design and implementation of a prototype of this system, {\em {\bf \system}}, which supports updating query plans at runtime to continually adapt to unanticipated changes in the volume and makeup of the input workload. Figure~\ref{fig:sonata-dynamiq} gives an overview of \system's architecture and shows its basic functionality in terms of first computing an initial query plan at compile time (using our boostrapping algorithms) and then dynamically updating this plan at runtime (using our runtime algorithms). This work makes the following concrete contributions:

\paragraph{Network Dynamics Characterization (Section~\ref{sec:background}).} 
We leverage packet traces from production traffic to better understand the limitations of static query plans. In particular, we use Sonata~\cite{sonata} as a use case and show that relying on static query plans can increase the amount of traffic sent to the stream processor by 3-4 orders of magnitude, which is of the same order as the stream processor's load without any query partitioning. We further show that static query plans are ill-suited to leverage the mix of increases and decreases in memory requirements that the different stateful operators experience over time. In contrast, query plans that can dynamically redistribute memory between different operators at runtime are better suited to make the best use of limited data-plane resources.

\ag{We need decouple Sonata-specific heuristics from more generalized takeaways. General takeaways: bootstrap, dynamic operator mapping. Sonata-specific contributions: TOM, slice-n-repeat (?), workload prediction, greedy operator mapping. Are any of these algorithms applicable for non-Sonata solutions (Marple/MAX-DP)? Our current plan is to argue that Sonata=iterative refinement. So, if we quantify the contributions of these algorithms w/o refinement, we can demonstrate their value. Clearly, we need to ignore TOM. It is too Sonata-specific. So far, the it looks like the current greedy solution does not works for MAX-DPs. What about the workload prediction? Does it performs reasonably well for FIX-REF? I remember that we discussed a while back that workload predictions for /32 were quite accurate. Maybe we want to quantify the performance of SnR and workload-pred. for FIX-REF, and also explore how to adapt the greedy algorithm for more effective dynamic operator mapping as well. That way we can make a stronger argument of how our contributions are decoupled from Sonata.}

\paragraph{Bootstrapping algorithms (Section~\ref{sec:bootstrap}).} 
To scale query execution, Sonata partitions the input queries between the switch and stream processor and also refines them over consecutive windows, enabling it to selectively spend resources on portions of traffic relevant to the input queries. Its query-planning decision entails: (1)~\textit{refinement plan}: how to iteratively refine each query, (2)~\textit{register sizing}: how to configure register sizes for stateful operators, and (3)~\textit{operator mappings}: how to map dataflow operators to stateful/stateless data structures in the data plane. Recognizing that it is not possible to change refinement plans and register sizes at runtime, it is of critical importance to be able to compute effective refinement plans and register sizes at compile-time. To this end, we present the design and implementation of two algorithms that compute initial refinement plans and register size configurations, respectively. We demonstrate that these algorithms have desirable properties, including the ability to find effective query plans for different input workloads and data-plane targets.

\paragraph{Runtime algorithms (Section~\ref{sec:runtime}).} 
We present the design and implementation of two runtime algorithms. The first algorithm considers an operator's past memory requirements and estimates that operator's required memory for the future window. The second algorithm uses these predicted values to compute new operator mappings. We demonstrate that these algorithms are practical in the sense that their combined overhead is minimal and well within the range of what \system's runtime requires. 
%of computing and updating operator mappings is marginal, compared to Sonata.

Our prototype augments Sonata's query-planner, runtime, and data plane driver modules, and we plan to open source our prototype. In Section~\ref{sec:implement}, we describe how \system leverages existing data-plane targets (e.g., Barefoot Tofino~\cite{tofino}) to enable updating operator mappings at runtime. In Section~\ref{sec:eval}, we use a set of realistic monitoring queries~\cite{sonata} as static query workload and publicly available real-world packet traces~\cite{caida15} as input workload to show that dynamic query planning as employed by \system reduces the stream processor's workload by two orders of magnitude compared static query planning used by Sonata.
% We also provide a detailed evaluation of which algorithmic components of \system are responsible for what portions of the observed improvement in performance. 

\ag{We need to rewrite this paragraph. It gives an impression that we are completely blank on handling dynamic queries, which is not true. We have some discussion on how DynamiQ can be extended to support dynamic queries in Section 8. We can consider moving this text to conclusion and merge it with text in Section 8 to make a more comprehensive argument on limitations of the current system, and how its design offers opportunities to handle dynamic queries as well. We can also refer to Newton here, and argue that Newton already instantiated some of these ideas. However, Newton is blank on how to make the operator mapping decisions, given query and workload dynamics.}
Note that like Sonata, \system is designed to run on a single switch, not across multiple switches, and assumes a fixed set of input queries (i.e., static query workload). Despite these current limitations, by supporting dynamic query planning, \system makes a critical contribution towards realizing the full promise of the next generation of hybrid network streaming analytics systems for scaling query execution to a level that full-fledged network automation will require in the future. 
% \rjh{This paragraph seems odd.  Why should the reader understand what ``single-node and requiring static query workloads'' means at this point? WW: changed phrasing -- related to Sonata wrt single-node issue and modified text wrt dynamic query workload}



% To fully benefit from the opportunities afforded by modern hardware-based network streaming analytics systems such as Sonata, they must formulate and employ query plans that are dynamic (\ie can change from one window to the next to adequately account for the differences in the makeup of the input workload), are practical (\ie can be efficiently computed), and can be implemented at runtime (\ie without disrupting normal switch operations and without knowledge of the future workload). \system satisfies these requirements and makes the following concrete contributions:
% \paragraph{Dynamic query plans as a pre-requisite for future hybrid streaming network analytics systems.} 2-3 sentences (Section 2).
% \paragraph{New algorithms for computing effective initial query plans.} 2-3 sentences of text (Section 3).
% \paragraph{Efficient algorithms for dynamic operator mapping at runtime.} 2-3 sentences (Section 4).
% \paragraph{Modular and extensible software architecture.} 2-3 sentences (Section 5).

% More concretely, we identify that changing refinement plan and register sizes over time is impractical. Thus, we first focus on developing bootstrapping algorithms that compute effective initial query plans, i.e., refinement plan and register sizes. We then focus on developing a learning model that uses the past cost values to predict future memory requirements for different operators---alleviating the need to make assumptions about the future traffic. We then take these predicted values as input to update operator mappings at runtime, ensuring efficient usage of data plane resources, and thus, reducing the load at the stream processor. 

%  Thus, dynamic query planning focuses on computing efficient initial query plans that



% 




% that is ``best" for a given window's workload in the sense that the plan minimizes the number of packets that cannot be processed in the data plane and must be sent to the stream processor. Serving as proof-of-concept, Sonata solves this optimization problem offline for a single training dataset and assumes that the resulting query plan is also effective for the workloads observed in future windows. 

% Query planning for Sonata deals with  the following questions: (1)~how to iteratively refine input queries, (2)~how to configure the packet-processing pipeline in the data plane (\eg size of hash tables used for stateful operations), and (3)~how to map Sonata's high-level dataflow operators to stateful/stateless data structures in the switch. 










%In this paper, we study the problem of dynamic query planning for modern network streaming analytics systems and focus in particular on the development of practical algorithms that we integrate into a production-ready network streaming analytics system. We present a prototype of this system, {\em {\bf \system}}, which supports updating query plans at runtime to adapt to changes in the volume and makeup of incoming traffic.  By supporting dynamic query planning, \system fully realizes the promise of hardware-based platforms for scaling query execution in the data plane. 

%In theory, query planning is concerned with a given set of queries and requires an understanding of how the traffic that is seen at a programmable data plane target during a given window gets mapped to a traffic workload that has to be processed by the stream processor because the query plan for that window cannot accommodate the execution of some dataflow operations associated with some of the queries in the data plane. We note that gaining an understanding of this mapping requires addressing two challenging problems that have not been widely studied in the past. TBD: (1) from traffic workload at the end of each window to corresponding cost matrix, (2) from measured past cost matrices to query plan for next window, (3) from new query plan to resulting workload at stream processor. 

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
% connect this with the trend of software-defined infrastructure ideas discussed by Amin in his keynote and how he emphasized the importance of taming the potential of hardware-based accelerators to address the scalability problem.
Networks supporting Internet-connected applications and devices have witnessed exponential growth in both scale and complexity. To effectively manage these networks, network operators need to detect a wide range of network events in (near) real time. As a result, network streaming analytics systems are now proliferating to run a wide range of queries for workloads up to billions of packets per second. Many of these systems (e.g., Sonata~\cite{sonata}) offload query execution to programmable data-plane targets (e.g., Barefoot Tofino~\cite{tofino}) to reduce the load on state-of-the-art stream processors (e.g., Apache Flink~\cite{flink}). For these systems, computing the right query plans that make the best use of limited hardware resources is critical. Without the right query plan, the promising hardware-based streaming analytics systems may not be deployable in production networks. 
% For example, network streaming analytics system, Sonata, is not capable of handling traffic dynamics. As a result, it misses out on opportunities to reduce the workload at the stream processor by multiple orders of magnitude. 

% narrow down the argument
To scale query execution, Sonata not only partitions the input queries between the switch and stream processor ({\em query partitioning}), but it also dynamically refines the input queries to selectively spend resources on portions of traffic relevant to the input query ({\em iterative refinement}). Therefore, the query planning process for systems similar to Sonata must answer the following questions: (1)~how should it refine each input query, (2)~how should it partition queries executing at different refinement levels, (3)~how should it configure the packet-processing pipeline in the data plane (e.g., size of hash tables used for stateful operations), and finally (4)~how should it map high-level dataflow operators to stateful/stateless data structures in the switch. To answer these questions, Sonata's query planner query planner solves an integer linear program (ILP) to determine a query plan for the given workload. Sonata solves this optimization problem only once and assumes that these query plans are effective for future workloads as well. However, we observed that's not the case. More concretely, we observe that the load at stream processor increases by 3-4 orders of magnitude if we don't update query plans over time, which is similar to load at stream processor without using data-plane targets for query execution. Thus, updating the query plans is critical to leverage the opportunities offered by harware-based targets. 
% \ag{the term {\em workload} is getting overloaded: workload at stream processor and workload for Sonata}

One approach can be to simply use Sonata's query planner for future windows. In theory, this approach is efficient in reducing the load at the stream processor, but it is not practical for three reasons: (1)~Sonata's query planning is NP-hard, and is not suited for real-time decision making, (2)~it requires a cost matrix (an estimate of the memory requirements for all stateful operators for all possible partitioning and refinement plans) for the future window as input, which is non-trivial, and (3)~it is agnostic to data-plane's reconfigurability constraints. More concretely, new plans require resizing the size of hash tables in the data plane, which requires taking the switch offline for few tens of seconds (disruptive). In general, the relatively large decision space and limited knowledge about the future workload, makes the problem of adapting query plans for dynamic workloads challenging. 

%\ag{TODO: refine this paragraph later.}
In this paper, we first decompose the query planning into three different sub-problems. First, we develop algorithms to compute query plans at the boot time, such that they help reduce the load at stream processor over time. Second, we develop machine-learning-based algorithm that output of queries from previous windows as input to predict the future workload at the end of each window. Finally, we develop an algorithm that uses the predicted workload as input to compute the query plan for the next window. We integrate all the individual algorithms into a production-ready network streaming analytics system, {\em {\bf \system}}, that updates the query plans at runtime---minimizing the load at stream processor over time. 

% \ag{TODO: use a uniform structure to make these three points}
% We present the following contributions:
% \begin{itemize}
%     \item {\em Bootstrapping Algorithms} (Section~\ref{sec:bootstrap}). Here, we first present the design of Bayesian Optimization (BO) algorithm to compute one-query-plan (OQP) that minimizes the maximum load at the stream processor over time. We then use this query plan to explore the design of an algorithm that computes both the bootstrapping refinement plan as well as the data-plane configuration. 
    
%     \item {\em Runtime Algorithms.} (Section~\ref{sec:runtime}). Here, we first characterize the spatial sparsity of the workload. We then leverage this sparsity to design a lightweight workload-prediction algorithm. We also present the design of a query-planning algorithm that computes the query plan at the end of every window. 
    
% \end{itemize}


% a new query-planning algorithm whose load reduction efficiency is close to theoretical optimal, while incurring significantly lower compute overhead, satisfying various data-plane reconfigurability constraints, and making the best use of limited knowledge of the future traffic. We developed new compilation techniques that are capable of making more efficient usage of limited resources and reconfigurability in the data plane. We have integrated these algorithms and compilation techniques with Sonata. We divide our efforts to make query planning more robust to traffic dynamics into three broader questions. 


% In the first case (Section~\ref{sec:bo}), we consider a setup where we do not change query plan over time. We also assume oracular knowledge of future workload. Given this knowledge, we explore the design of an algorithm that can compute one-query-plan (OQP) that minimizes the maximum load at the stream processor over time. To this end, we first present the formulation of an optimal query planning problem for this setup, and then present an algorithm that uses Bayesian Optimization (BO) to compute this (near) optimal query plan. We then quantify the performance of this solution to identify the lower bound of solutions that do not dynamically update the query plans over time. 
% % We also explore the relationship between this performance gap and data-plane resources. We use this understanding to compute a configuration where this gap is highest. 

% In the second case (Section~\ref{sec:pilp}), we consider a setup where we can change the query plans over time. We still assume oracular knowledge of future workload. As we discussed earlier, both reconfiguring the packet-processing pipeline as well as changing refinement plans over time is impractical. Thus, the new query plans can only differ in their partitioning plan as well as how they map high-level dataflow operators to stateless/stateful data structures in the data plane. In this case, we also need to compute the appropriate data-plane configurations and refinement plans at the start such that they enable efficient handling of traffic dynamics over time. To this end, we first formulate the bootstrapping problem, and show that it is NP-hard. We then present observations that motivate the design of heuristics-based algorithm for computing both data-plane configurations as well as refinement plans. More concretely, we demonstrate how these bootstrapping configurations are related to OQPs. 

% Next, we explore the problem of computing query plans at runtime. Again, we show that the problem is NP-hard, which is problematic as we need to compute a solution in near real time. To address this problem, we map this problem to a weighted stable matching problem and design a heuristic-based algorithm to compute (near) optimal query plans at runtime. 

% In the third case (Section~\ref{sec:lstm}), we consider the most realistic setup, where we can change query plans over time and we do not have oracular knowledge of the future workload. In this case, we first need to predict the future workload and then apply the above heuristics-based query-planning algorithm for the predicted workload. Note, that now in addition to computing the query plan, we also need to compute the workload for future workload at runtime. For this problem, we first characterize the spatial sparsity of the workload. We then leverage this sparsity to design a lightweight workload-prediction algorithm. Overall, this final case leverages the OQPs (case~1) to bootstrap the query plans (case~2). At the end of each window, it uses workload-prediction algorithm to estimate the workload for next window (case~3), and then uses heuristics-based query-planning algorithm (case~2) to compute the query plan for this window. 

% \ag{TODO: approach, key observation, ideas, etc.}

% We present the following contributions. 

% \smartparagraph{Characterization}


% \smartparagraph{Algorithm}

% \smartparagraph{Implementation}


%  This demand  has motivated the development of various network-streaming analytics systems that are both flexible and scalable. One such system, Sonata~\cite{sonata-hotnets}, strikes a good balance between flexibility and scale. It lets network operators express a wide range of network analytics tasks as dataflow queries over arbitrary packet tuples---enabling flexibility; and uses PISA-based targets to execute a subset of these queries in the data plane before sending it to a userspace stream processor---enabling scalability.

% Compared to the general-purpose processors (e.g., X-86), which are typically used for the streaming-analytics tasks, data-plane targets (e.g., Barefoot Tofino~\cite{tofino}) have limited compute and memory resources and are hard to reconfigure at the runtime. Thus, a query planner is required to decide how to make the best use of limited in-network resources over time. In case of Sonata, its query planner solves an integer linear program (ILP) to determine a query plans for the given workload. This plan specifies how to iteratively refine input queries and partition them between the data-plane and user-space targets. From the previous work~\cite{sonata-hotnets}, it is clear how Sonata's query planner will perform if the given workload does not change over time. However, given the dynamic nature of network traffic in production settings, the workload for the query planner changes over time. As a result, it is not clear how Sonata-like network streaming analytics systems will perform in production settings. Thus, it is critical to first understand how the existing systems handle traffic dynamics and how they can be improved to make them robust for real-world operations.










==> related.tex <==
\section{Related Work}
\label{sec:related}


% \smartparagraph{Network telemetry.} Existing telemetry systems that process
% all packets at the stream processor such as Chimera~\cite{chimera},
% Gigascope~\cite{gigascope}, OpenSOC~\cite{opensoc}, and NetQRE~\cite{netqre}
% can express a range of queries but can only support lower packet rates because the stream processor ultimately processes all results. These systems
% also require deploying and configuring a collection infrastructure to capture
% packets from the data plane for analysis, incurring significant bandwidth
% overhead.  These systems can benefit from horizontally scalable stream
% processors such as Spark Streaming~\cite{dstream} and Flink~\cite{flink}, but
% they also face scaling limitations due to packet parsing and cluster
% coordination~\cite{osoc-scale}.

% Everflow~\cite{everflow}, UnivMon~\cite{univmon}, OpenSketch~\cite{opensketch},
% and Marple~\cite{marple} rely on programmable switches to execute queries entirely 
% in the data plane. These systems can process queries at line rate but can only support 
% queries that can be implemented on switches.
% Trumpet~\cite{trumpet} and Pathdump~\cite{pathdump} 
% offload query processing to end-hosts (VMs in data center networks) but not to 
% switches. Our previous work~\cite{sonata-hotnets} proposed a telemetry system that
% partitions a single query across a stream processor and switch, but it only considers 
% switches with fixed-function chipsets, and requires the network operators to specify the 
% refinement and partitioning plans manually. In contrast, \system supports programmable 
% switches and employs a sophisticated query planner to automatically partition and refine 
% multiple queries. 
% %We also quantify the performance gains and overhead with realistic packet 
% %traces and a programmable hardware switch.

% \if 0
% \begin{table}[t]
% \smallskip\noindent
% \begin{footnotesize}
% \centering
% \resizebox{.9\linewidth}{!}{
% \newcommand\items{5}   %Number of classes
% \arrayrulecolor{black} %Table line colors
% \noindent
% \begin{tabular}{|c|*{\items}{E}|}
% \hline
% %\multicolumn{1}{|c}{} &
% \multicolumn{1}{|c|}{} &
% \arot{Granularity} &
% \arott{Complexity} &
% \arot{Filtering} &
% \arot{Aggregation} &
% \arott{Refinement} \\ 
% \hline
% %\multirow{3}{*}{Sec~\ref{sec:gp-sols}}
% OpenSOC~\cite{opensoc} & 1 & 1  & 0 & 0 & 0 \\
% %\multirow{2}{*}{\rotatebox[origin=c]{90}{Sec~\ref{ssec:gp-sols}}} 
% Chimera~\cite{chimera} & 1 & 1 & 0 & 0 & 0 \\ 
% NetQRE~\cite{netqre} & 1 & 1 & 0 & 0 & 0 \\ 
% Gigascope~\cite{gigascope} & 1 & 1 & 150 & 150 & 0 \\ 
% \hline
% Marple~\cite{marple} & 0 & 150 & 1 & 1 & 0 \\ 
% %\multirow{3}{*}{\rotatebox[origin=c]{90}{Sec~\ref{ssec:dp-sols}}} 
% Everflow~\cite{everflow} & 0 & 0 & 1 & 0 & 0 \\
% Trumpet~\cite{trumpet} & 0 & 0 & 1 & 1 & 0 \\ 
% OpenSketch~\cite{opensketch} & 0 & 0 & 1 & 1 & 0 \\
% UnivMon~\cite{univmon} & 0 & 0 & 1 & 1 & 0 \\ 
% DREAM~\cite{dream} & 0 & 0 & 1 & 1 & 1 \\ 
% \hline
% \textbf{Sonata} & 1 & 1 & 1 & 1 & 1 \\
% \hline
% \end{tabular}
% }
% \caption{Current streaming network telemetry approaches. Darker shading
% indicates full support of a feature while lighter shading indicates partial
% or limited support.}
% \label{tab:design-space}
% \end{footnotesize}
% \end{table}
% \fi


% \smartparagraph{Query planning.}
% Database research has explored query planning and optimization 
% extensively~\cite{polychroniou2014track, mullin1990optimal, catalyst}. 
% Gigascope performs query partitioning to minimize the
% data transfer from the capture card to the stream processor~\cite{gigascope}. 
% Sensor networks have explored the query partitioning problems that are similar
% to those that \system 
% faces~\cite{polychroniou2014track,mullin1990optimal,catalyst,
%                 Madden.OSDI02,tinydb,Srivastava.PODS05}.  However, these systems face different optimization problems because
% they typically involve lower traffic rates and involve special-purpose
% queries. Path Queries~\cite{pathquery} and
% SNAP~\cite{snap} facilitate network-wide queries that execute across multiple
% switches; in contrast, \system currently only compiles queries to a single
% switch, but it addresses a complementary set of problems, such as unifying
% data-plane and stream-processing platforms to support richer queries and
% partitioning sets of queries across a data-plane switch and a stream processor.

% \smartparagraph{Query-driven dynamic refinement.}
% Autofocus~\cite{autofocus}, ProgME~\cite{progme}, and
% DREAM~\cite{dream}, SCREAM~\cite{scream}, MULTOPS~\cite{multops}, 
% and HHH~\cite{jose2011online} all iteratively zoom in on traffic of interest. 
% These systems either do not apply to
% streaming data (\eg, ProgME requires multiple passes over the data~\cite{progme}),
% they use a static refinement plan for all queries (\eg, HHH 
% zooms in one bit at a time), or they do not satisfy general queries on network traffic (\eg, MULTOPS is specifically designed for bandwidth attack detection). 
% These approaches all rely on general-purpose CPUs to process the data-plane output, but none of them permit additional parsing, joining, or aggregation at the stream processor, as \system does.



